OpenMatch: Open-set Consistency Regularization for Semi-supervised Learning with Outliers

Semi-supervised learning (SSL) is an effective means to leverage unlabeled data to improve a model's performance. Typical SSL methods like FixMatch assume that labeled and unlabeled data share the same label space. However, in practice, unlabeled data can contain categories unseen in the labeled set, i.e., outliers, which can significantly harm the performance of SSL algorithms. To address this problem, we propose a novel Open-set Semi-Supervised Learning (OSSL) approach called OpenMatch. Learning representations of inliers while rejecting outliers is essential for the success of OSSL. To this end, OpenMatch unifies FixMatch with novelty detection based on one-vs-all (OVA) classifiers. The OVA-classifier outputs the confidence score of a sample being an inlier, providing a threshold to detect outliers. Another key contribution is an open-set soft-consistency regularization loss, which enhances the smoothness of the OVA-classifier with respect to input transformations and greatly improves outlier detection. OpenMatch achieves state-of-the-art performance on three datasets, and even outperforms a fully supervised model in detecting outliers unseen in unlabeled data on CIFAR10.

==> algo_old.tex <==

\begin{algorithm}[!tp]

1: {\bfseries Input} Batch of labeled examples and their one-hot labels $\mathcal{X} = \big((x_b, p_b); b \in (1, \ldots, B)\big)$, batch of unlabeled examples $\mathcal{U} = \big(u_b; b \in (1, \ldots, B)\big)$. batch of pseudo-known unlabeled examples $\mathcal{K} = \emptyset$. 

Model's parameters, $w$, learning rate $\eta$, epoch \rev{$T_{fix}$}{$E_{warm-up}$} and \rev{$T_{\max}$}{$E_{\max}$}, iteration $N_{\max}$, trade-off parameters, $\lambda_1, \lambda_2, \lambda_3$;

\For{$T = 1,2,\dots,T_{\max}$}{

	2: {\bfseries Shuffle} training set $\mathcal{X}, \mathcal{U}$; \hfill //
	
	\For{$N = 1,\dots,N_{\max}$}
	{	3: {\bfseries Input} $\hat{x}_b, \hat{u}_{b1}, \hat{u}_{b2} =  \augment(x_b), \augment(u_b), \augment(u_b)$; \hfill //augment images
		%3: {\bfseries Fetch} mini-batch $\bar{\mathcal{D}}$ from $\mathcal{D}$;
		
		4: {\bfseries Compute} $L_{all} = L_s(\hat{x}_b, y_b) + \lambda_1 L_{em} ( \hat{u}_{b1}) + \lambda_2 L_{oc}( \hat{u}_{b1},  \hat{u}_{b2})$; \hfill //Compute loss 
		
		\If {$T > T_{fix}$}{
		5: {\bfseries Compute} $L_{all} \mathrel{+}= \lambda_3 L_{fix}(\hat{k}_{b})$  ($\hat{k}_{b} \sim \mathcal{K}$) ; \hfill //FixMatch for pseudo-known samples. 
		
		}
		6: {\bfseries Update} $w = w - \eta\nabla L_{all}$; \hfill //update weights;
	}
    \If {$T \geq T_{fix}$}{
		7: {\bfseries Update} $\mathcal{K} = \select(w, \mathcal{U})$; \hfill //Select pseudo-known samples for FixMatch;
	}	
}
8: {\bfseries Output $w$.}
\caption{OpenMatch Algorithm.}
\label{alg:openmatch}
\end{algorithm}


==> method_old.tex <==
\section{OpenMatch}
OpenMatch is a combination of three approaches:\rev{ one-vs-all classifier based open-set classification, open-set soft-consistency regularization, and FixMatch}{(1) one-vs-all classifier based open-set classification to detect outliers, (2) open-set soft-consistency regularization to improve the smoothness of the model, and (3) FixMatch for SSL learning objectives with in-liers}. Its main technical novelty comes from the soft-consistency regularization as well as \rev{the way of unifying the approaches}{unified framework for OSSL}. 
The one-vs-all classifies trained with soft-regularization effectively separate known and unknown samples, and FixMatch is applied only to pseudo-known samples. 
We first describe how to train one-vs-all classifiers~\cite{saito2021ovanet} before describing the details of our framework. 

\subsection{Problem setting and One-vs-All Network}
\textbf{Problem Setting.}
For a L-class classification problem, let $\mathcal{X}=\left\{\left(x_{b}, {y_{b}}\right) : b \in (1,... B)\right\}$ be a \rev{batch}{set} of B labeled examples, where $x_b$ are the training examples and $y_b \in (1,... L)$ are the corresponding labels. Let $\mathcal{U}=\left\{(u_{b}) : b \in (1,... \mu B)\right\}$ be a \rev{batch}{set} of $\mu B$ unlabeled examples where $\mu$ is a hyperparameter that determines the relative sizes of $\mathcal{X}$ and $\mathcal{U}$. SSL assumes the label space of $\mathcal{U}$ and $\mathcal{X}$ is the same whereas OSSL hypothesizes that of $\mathcal{U}$ includes labels absent in $\mathcal{X}$. The goal of OSSL is to classify known samples into the correct classes while learning representations effective to detect the outliers. \donghyun{Our model has three components: (1) shared feature extractor $F(\cdot)$, (2) open-set classifier consisted of one-vs-all sub-classifiers $O^{j}, j \in \{1, . . . , L\}$ for out-liers, and (3) closed-set classifier $C(\cdot)$ for in-liers.}


\textbf{One-vs-All Classifier.} For open-set~\cite{saito2018open} or universal domain adaptation~\cite{UDA_2019_CVPR} \donghyun{scenarios}, Saito~\etal~\cite{saito2021ovanet} propose to train one-vs-all classifiers to detect out-lier samples of an unlabeled target domain. They aim to learn a boundary between in-liers and outliers for each class. The open-set classifiers consist of $L$ sub-classifiers, i.e., $O^{j}, j \in \{1, . . . , L\}$. Each \donghyun{sub-}classifier is trained to distinguish if the sample is an in-lier for the corresponding class. The sub-classifier outputs a 2-dimensional vector, where each dimension shows the probability of a sample being an in-lier and outlier respectively. Then, the \donghyun{sub-}classifier $O^{j}$ is trained such that the data from class $j$ is treated as positives, and the data from all the other classes is treated as negatives \donghyun{(\ie, one-vs-all classifier)}. The key is that \rev{the classifiers}{each sub-classifier} can output the distance representing how the input is far from \rev{each class}{its own class}. Therefore, the classifiers are effective to identify unlabeled unknown samples. Saito \etal introduce hard-negative classifier sampling technique to effectively learn the threshold~\cite{saito2021ovanet}. Since the details are not the scope of this work, we explain them in the appendix. Given a shared feature extractor, the model has two heads: closed-set classifier outputs label-distribution of known classes, open-set classifier outputs anomaly score for each class. Then, for labeled samples, the objective consists of two terms: closed-set classification loss, which is a standard cross-entropy loss, and open-set classification loss. We summarize the supervised loss for the labeled samples, $\left(x_{b}, {y_{b}}\right)$ as $L_s(x_{b}, y_b)$. 



\textbf{Open-set Entropy Minimization.} 
For unlabeled samples, they apply entropy minimization with respect to the one-vs-all classifiers as denoted as $L_{em}(u_{b})$. The separation between known and unknown samples is enhanced through the minimization of the unsupervised loss. In their problem setting, they employ a model pre-trained on ImageNet~\cite{imagenet}, which extracts highly discriminative features, and the known and unknown samples are well-separated even before fine-tuning. However, we aim to train a model to learn representations separating known and unknown samples from scratch.

%We call the categories unique to $\mathcal{U}$ ``unknown'' or ``novel'' categories. 
%The goal of OSSL is to label the target samples with either one of the $L_s$ labels or the ``unknown'' label. We train the model on $\mathcal{D}_{s} \cup \mathcal{D}_{t}$ and evaluate on $ \mathcal{D}_{t}$. To handle the open-set classification, we introduce both open-set classifiers, $O$, and a closed-set classifier, $C$. $C$ is trained to classify source samples with a standard classification loss while $O$ is trained with \textit{hard negative classifier sampling} explained below. $C$ is used to identify a nearest known class while $O$ is used to determine whether the sample is known or unknown.
\input{figures/openset}
\subsection{Soft Open-set Consistency Regularization}
We describe the difference between SSL and OSSL in Fig.~\ref{fig:comparison}.
In SSL, the hard consistency loss such as pseudo-labeling can be effective to propagate label information from labeled to unlabeled samples. The open-set entropy minimization above is also considered to be a variant of the hard consistency since it is minimized if the predicted output class distribution is one-hot.
Through the hard consistency loss, unlabeled samples are supposed to get training signals from neighboring labeled samples. 
By contrast, in OSSL, since any novel samples are not assigned labelss, neighboring labeled samples are far from the novel samples, which makes the hard-labeling unreliable and unsupervised training signals can be noisy. Therefore, it is necessary to provide smoothing to the decision boundary of the open-set classifier. The smoothing will be effective to propagate less noisy training signals for the open-set entropy minimization.

Specifically, our soft consistency regularization enhances the smoothness of the open-set classifier on unlabeled data over data augmentations $\mathcal{T}$. We obtain two different views of $u_b$, $\mathcal{T}_1(u_b)$ and $\mathcal{T}_2(u_b)$, where $\mathcal{T}_{1}$ and $\mathcal{T}_{2}$ are data augmentation functions stochastically sampled from $\mathcal{T}$.
%Specifically, our soft consistency regularization enhances smoothness with respect to different data augmentations. 
Let $p_{o}(t | \mathcal{T}_1(u_b))$ be the output logits from the open-set classifier of $\mathcal{T}_1(u_b)$. We encourage the consistency of the output logits over the different data augmnetations $\mathcal{T}$ to enhance the smoothness. Finally we minimize the following loss:

\begin{equation}
    \mathcal{L}_{oc} = \frac{1}{B}\sum_{b=1}^{B}|p_{o}(t | \mathcal{T}_{1}(u_b)) - p_{o}(t |\mathcal{T}_{2}(u_b))|^{2}.
    \label{eq:oc}
\end{equation}

Note that the key of the regularization is applying the consistency in a soft manner. 

%Let $p_{o}(t | \alpha(u_b))$ be the output logits of the open-set classifier, where $\alpha$ denote the data augmentation function stochastically sampled from $\mathrm{A}$. Then, we compute the following loss to see the smoothness for different data augmentations:

%\begin{equation}
%    L_{oc} = \frac{1}{B}\sum_{b=1}^{B}|p_{o}(t | \alpha(u_b)) - p_{o}(t |\hat{\alpha}(u_b))|^{2}, 
%\end{equation}
%where both $\alpha$ and $\hat{\alpha}$ are stochastically sampled from $\mathrm{A}$. 

%\donghyun{(suggestion for the above paragraph) Specifically, we enhance the smoothness of the open-set classifier by soft consistency regularization on an unlabeled data $u_b$ over data augmentations $\mathcal{T}$. We obtain two different views of $u_b$, $T_1(u_b)$ and $T_2(u_b)$, where $T_{1}$ and $T_{2}$ are independent data augmentation functions stochastically sampled from $\mathcal{T}$. Let $p_{o}(t | T_1(u_b))$ be the output logits from the open-set classifier of $T_1(u_b)$. We encourage the consistency of the output logits over the different data augmnetations $\mathcal{T}$ to enhance the smoothness. Finally we minimize the following loss:

%\begin{equation}
%    L_{oc} = \frac{1}{B}\sum_{b=1}^{B}|p_{o}(t | T_{1}(u_b)) - p_{o}(t |T_{2}(u_b))|^{2}, 
%\end{equation}
%}



%See Fig. 
% \input{algo}
\input{algo2}
\subsection{OpenMatch}
The unsupervised losses for open-set classifier are effective to detect outliers. However, the losses are not sufficient to correctly classify unlabeled in-liers. Therefore, we propose to introduce semi-supervised learning loss for unlabeled samples classified as in-liers. We introduce FixMatch~\cite{sohn2020fixmatch} since it is a simple, yet very strong SSL method. After training a model for $E_{fix}$ epochs with $L_{em}$, $L_{oc}$, and $L_{s}$, we classify unlabeled samples into known or unknown in every epoch. 
In  Alg.~\ref{alg:openmatch}, $\select(w, \mathcal{U})$ denotes the process of classifying unlabeled samples given model's parameter $w$ and unlabeled data.
Then, FixMatch loss, $L_{fm}$, is computed only for the pseudo-known samples to optimize a model. We call the whole framework {\it OpenMatch}. 
The following is the resulting objective:
\begin{equation}
    L_{s} + \lambda_{em} L_{em} + \lambda_{oc} L_{oc} + \lambda_{fm} L_{fm},
\end{equation}
where $\lambda_em$,  $\lambda_oc$ and  $\lambda_f$ control the trade-off for each objective.
$\lambda_em$ is set 0.1 in all experiments. 
Note that $\lambda_f$ is set 0 before $E_{fix}$ epochs and is set as 1 for all experiments. 
The whole algorithm is described in Alg.~\ref{alg:openmatch}. 


